Outage performance analysis of RIS-assisted UAV wireless systems under disorientation and misalignment

In this paper, we analyze the performance of a reconfigurable intelligent surface (RIS)-assisted unmanned aerial vehicle (UAV) wireless system that is affected by mixture-gamma small-scale fading, stochastic disorientation, and misalignment, as well as transceivers hardware imperfections. First, we statistically characterize the end-to-end channel for both cases, i.e., in the absence as well as in the presence of disorientation and misalignment, by extracting closed-form formulas for the probability density function (PDF) and the cumulative distribution function (CDF). Building on the aforementioned expressions, we extract novel closed-form expressions for the outage probability (OP) in the absence and the presence of disorientation and misalignment as well as hardware imperfections. In addition, high signal-to-noise ratio OP approximations are derived, leading to the extraction of the diversity order. Finally, an OP floor due to disorientation and misalignment is presented.

==> 1.5. arxiv/images/organization.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,799); %set diagram left start at 0, and has height of 799
	
	%Straight Lines [id:da7549665141364654] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (50,21) -- (50,760) ;
	%Straight Lines [id:da47625167392970713] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (49,21) -- (86,21) ;
	\draw [shift={(89,21)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da14186589472175903] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (51,111) -- (88,111) ;
	\draw [shift={(91,111)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9483543763704907] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (51,140) -- (88,140) ;
	\draw [shift={(91,140)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da7917046674146371] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (51,170) -- (88,170) ;
	\draw [shift={(91,170)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da49631263983654694] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,200) -- (108,200) ;
	\draw [shift={(111,200)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da704360701576451] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,170) -- (71,381) ;
	%Straight Lines [id:da45229232300561106] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,229) -- (128,229) ;
	\draw [shift={(131,229)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da03584291262622097] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,200) -- (91,350) ;
	%Straight Lines [id:da616440142730736] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (92,260) -- (129,260) ;
	\draw [shift={(132,260)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da11951286587293786] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,260) -- (112,321) ;
	%Straight Lines [id:da27642545962354803] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,291) -- (149,291) ;
	\draw [shift={(152,291)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da5459855164810739] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,321) -- (149,321) ;
	\draw [shift={(152,321)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da5348702022757221] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,350) -- (127,350) ;
	\draw [shift={(130,350)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9867014456859513] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,381) -- (108,381) ;
	\draw [shift={(111,381)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6418925655118273] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,409) -- (128,409) ;
	\draw [shift={(131,409)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9876986683837687] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,380) -- (91,530) ;
	%Straight Lines [id:da8287168204190516] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (92,440) -- (129,440) ;
	\draw [shift={(132,440)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9576983292731358] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,440) -- (112,501) ;
	%Straight Lines [id:da6803705166706564] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,471) -- (149,471) ;
	\draw [shift={(152,471)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da3190777351415839] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,501) -- (149,501) ;
	\draw [shift={(152,501)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da04645716603992289] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,530) -- (127,530) ;
	\draw [shift={(130,530)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da999392842419778] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (50,561) -- (87,561) ;
	\draw [shift={(90,561)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da04270397591269859] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (70,583) -- (107,583) ;
	\draw [shift={(110,583)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da13839239630828648] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,612) -- (127,612) ;
	\draw [shift={(130,612)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9486747809556244] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,583) -- (90,643) ;
	%Straight Lines [id:da36389262070872097] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,643) -- (127,643) ;
	\draw [shift={(130,643)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da7501450490403929] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (70,561) -- (70,670) ;
	%Straight Lines [id:da11114295170924793] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (70,670) -- (107,670) ;
	\draw [shift={(110,670)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da35497592028348324] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,699) -- (127,699) ;
	\draw [shift={(130,699)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6435599189355405] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,670) -- (90,730) ;
	%Straight Lines [id:da0883718619590077] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,730) -- (127,730) ;
	\draw [shift={(130,730)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6124523428698243] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (50,760) -- (87,760) ;
	\draw [shift={(90,760)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da8997117662877758] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,21) -- (71,81) ;
	%Straight Lines [id:da8859923266700584] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,50) -- (108,50) ;
	\draw [shift={(111,50)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6960125977451803] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,81) -- (108,81) ;
	\draw [shift={(111,81)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	
	% Text Node
	\draw (167.04,19.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. I - Introduction}};
	% Text Node
	\draw (177.04,109.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. II - System model}};
	% Text Node
	\draw (261.04,139.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. III - E2e channel statistical characterization}};
	% Text Node
	\draw (204.04,169.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. IV - Performance analysis}};
	% Text Node
	\draw (222.04,199.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. IV-A - Ideal RF front-end}};
	% Text Node
	\draw (249.04,228.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A1 - Instantaneous SNR}};
	% Text Node
	\draw (195.04,259.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A2 - OP}};
	% Text Node
	\draw (296.04,289.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {Without disorientation and misalignment};
	% Text Node
	\draw (286.04,319.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {With disorientation and misalignment};
	% Text Node
	\draw (232.04,349.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A3 - Diversity order}};
	% Text Node
	\draw (238.04,379.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. IV-B - Non-ideal RF front-end}};
	% Text Node
	\draw (255.04,408.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A2 - Instantaneous SDNR}};
	% Text Node
	\draw (195.04,439.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A2 - OP}};
	% Text Node
	\draw (296.04,469.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {Without disorientation and misalignment};
	% Text Node
	\draw (286.04,499.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {With disorientation and misalignment};
	% Text Node
	\draw (232.04,529.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A3 - Diversity order}};
	% Text Node
	\draw (199.04,558.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. V - Results \& discussion}};
	% Text Node
	\draw (220.04,582.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. V-A - Ideal RF front-end}};
	% Text Node
	\draw (315.04,613) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-A1 - }Without disorientation and misalignment};
	% Text Node
	\draw (305.04,643) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-A2 - With} disorientation and misalignment};
	% Text Node
	\draw (236.04,671.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. V-B - Non-ideal RF front-end}};
	% Text Node
	\draw (315.04,700) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-B1 - }Without disorientation and misalignment};
	% Text Node
	\draw (305.04,730) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-B2 - With} disorientation and misalignment};
	% Text Node
	\draw (173.04,761.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. VI - Conclusions}};
	% Text Node
	\draw (237.04,49.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. I-A - Novelty and contribution}};
	% Text Node
	\draw (247.04,80.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. I-B - Organization and notations}};
	
	
\end{tikzpicture}


==> images/organization.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,799); %set diagram left start at 0, and has height of 799
	
	%Straight Lines [id:da7549665141364654] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (50,21) -- (50,760) ;
	%Straight Lines [id:da47625167392970713] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (49,21) -- (86,21) ;
	\draw [shift={(89,21)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da14186589472175903] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (51,111) -- (88,111) ;
	\draw [shift={(91,111)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9483543763704907] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (51,140) -- (88,140) ;
	\draw [shift={(91,140)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da7917046674146371] 
	\draw [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (51,170) -- (88,170) ;
	\draw [shift={(91,170)}, rotate = 180] [color={rgb, 255:red, 74; green, 74; blue, 74 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da49631263983654694] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,200) -- (108,200) ;
	\draw [shift={(111,200)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da704360701576451] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,170) -- (71,381) ;
	%Straight Lines [id:da45229232300561106] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,229) -- (128,229) ;
	\draw [shift={(131,229)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da03584291262622097] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,200) -- (91,350) ;
	%Straight Lines [id:da616440142730736] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (92,260) -- (129,260) ;
	\draw [shift={(132,260)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da11951286587293786] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,260) -- (112,321) ;
	%Straight Lines [id:da27642545962354803] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,291) -- (149,291) ;
	\draw [shift={(152,291)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da5459855164810739] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,321) -- (149,321) ;
	\draw [shift={(152,321)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da5348702022757221] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,350) -- (127,350) ;
	\draw [shift={(130,350)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9867014456859513] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,381) -- (108,381) ;
	\draw [shift={(111,381)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6418925655118273] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,409) -- (128,409) ;
	\draw [shift={(131,409)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9876986683837687] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (91,380) -- (91,530) ;
	%Straight Lines [id:da8287168204190516] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (92,440) -- (129,440) ;
	\draw [shift={(132,440)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9576983292731358] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,440) -- (112,501) ;
	%Straight Lines [id:da6803705166706564] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,471) -- (149,471) ;
	\draw [shift={(152,471)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da3190777351415839] 
	\draw [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (112,501) -- (149,501) ;
	\draw [shift={(152,501)}, rotate = 180] [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da04645716603992289] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,530) -- (127,530) ;
	\draw [shift={(130,530)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da999392842419778] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (50,561) -- (87,561) ;
	\draw [shift={(90,561)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da04270397591269859] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (70,583) -- (107,583) ;
	\draw [shift={(110,583)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da13839239630828648] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,612) -- (127,612) ;
	\draw [shift={(130,612)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da9486747809556244] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,583) -- (90,643) ;
	%Straight Lines [id:da36389262070872097] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,643) -- (127,643) ;
	\draw [shift={(130,643)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da7501450490403929] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (70,561) -- (70,670) ;
	%Straight Lines [id:da11114295170924793] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (70,670) -- (107,670) ;
	\draw [shift={(110,670)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da35497592028348324] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,699) -- (127,699) ;
	\draw [shift={(130,699)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6435599189355405] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,670) -- (90,730) ;
	%Straight Lines [id:da0883718619590077] 
	\draw [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (90,730) -- (127,730) ;
	\draw [shift={(130,730)}, rotate = 180] [color={rgb, 255:red, 5; green, 34; blue, 68 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6124523428698243] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (50,760) -- (87,760) ;
	\draw [shift={(90,760)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da8997117662877758] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,21) -- (71,81) ;
	%Straight Lines [id:da8859923266700584] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,50) -- (108,50) ;
	\draw [shift={(111,50)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	%Straight Lines [id:da6960125977451803] 
	\draw [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (71,81) -- (108,81) ;
	\draw [shift={(111,81)}, rotate = 180] [color={rgb, 255:red, 51; green, 51; blue, 50 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
	
	% Text Node
	\draw (167.04,19.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. I - Introduction}};
	% Text Node
	\draw (177.04,109.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. II - System model}};
	% Text Node
	\draw (261.04,139.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. III - E2e channel statistical characterization}};
	% Text Node
	\draw (204.04,169.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. IV - Performance analysis}};
	% Text Node
	\draw (222.04,199.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. IV-A - Ideal RF front-end}};
	% Text Node
	\draw (249.04,228.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A1 - Instantaneous SNR}};
	% Text Node
	\draw (195.04,259.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A2 - OP}};
	% Text Node
	\draw (296.04,289.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {Without disorientation and misalignment};
	% Text Node
	\draw (286.04,319.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {With disorientation and misalignment};
	% Text Node
	\draw (232.04,349.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A3 - Diversity order}};
	% Text Node
	\draw (238.04,379.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. IV-B - Non-ideal RF front-end}};
	% Text Node
	\draw (255.04,408.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A2 - Instantaneous SDNR}};
	% Text Node
	\draw (195.04,439.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A2 - OP}};
	% Text Node
	\draw (296.04,469.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {Without disorientation and misalignment};
	% Text Node
	\draw (286.04,499.5) node  [color={rgb, 255:red, 36; green, 74; blue, 119 }  ,opacity=1 ] [align=left] {With disorientation and misalignment};
	% Text Node
	\draw (232.04,529.5) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. IV-A3 - Diversity order}};
	% Text Node
	\draw (199.04,558.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. V - Results \& discussion}};
	% Text Node
	\draw (220.04,582.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. V-A - Ideal RF front-end}};
	% Text Node
	\draw (315.04,613) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-A1 - }Without disorientation and misalignment};
	% Text Node
	\draw (305.04,643) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-A2 - With} disorientation and misalignment};
	% Text Node
	\draw (236.04,671.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. V-B - Non-ideal RF front-end}};
	% Text Node
	\draw (315.04,700) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-B1 - }Without disorientation and misalignment};
	% Text Node
	\draw (305.04,730) node   [align=left] {\textcolor[rgb]{0.02,0.13,0.27}{Sec. V-B2 - With} disorientation and misalignment};
	% Text Node
	\draw (173.04,761.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. VI - Conclusions}};
	% Text Node
	\draw (237.04,49.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. I-A - Novelty and contribution}};
	% Text Node
	\draw (247.04,80.5) node   [align=left] {\textcolor[rgb]{0,0,0}{Sec. I-B - Organization and notations}};
	
	
\end{tikzpicture}

